A Foundation for Synthetic Stone Duality

The language of homotopy type theory has proved to be appropriate as an internal language for various higher toposes, for example with Synthetic Algebraic Geometry for the Zariski topos. In this paper we apply such techniques to the higher topos corresponding to the light condensed sets of Dustin Clausen and Peter Scholze. This seems to be an appropriate setting to develop synthetic topology, similar to the work of Mart\'in Escard\'o. To reason internally about light condensed sets, we use homotopy type theory extended with 4 axioms. Our axioms are strong enough to prove Markov's principle, LLPO and the negation of WLPO. We also define a type of open propositions, inducing a topology on any type. This leads to a synthetic topological study of (second countable) Stone and compact Hausdorff spaces. Indeed all functions are continuous in the sense that they respect this induced topology, and this topology is as expected for these classes of types. For example, any map from the unit interval to itself is continuous in the usual epsilon-delta sense. We also use the synthetic homotopy theory given by the higher types of homotopy type theory to define and work with cohomology. As an application, we prove Brouwer's fixed-point theorem internally.

==> BinaryRep.tex <==
In this section we will introduce the unit interval $I$ as compact Hausdorff space. 
The definition is based on \cite{Bishop}. 
%We will then calculate the cohomology of $I$. 
%For a proof that the unit interval corresponds to the definition using Cauchy sequences, 
%we refer to the appendix. 


%\input{Interval/CauchySequences}
%------------------content of file BinaryClosedEquivalence.tex...
%We want to show that the interval of Cauchy reals is Compact Hausdorff. 
%Informally, to any binary sequence $\alpha : \N \to 2$, 
%we can associate a Cauchy sequence 
%$cs(\alpha)$, given by 
%\begin{equation}\label{eqnBinaryEncode}
%  (cs(\alpha))_n = \sum\limits_{i = 0 }^n \frac {\alpha(i)}{2^{i+1}}
%\end{equation}
%and we are going to give a closed relation on Cantor space such that 
%two binary sequences are equivalent iff they correspond to the same Cauchy reals. 
\begin{example}
  Let $n:\N$, we denote $C_n = 2[n]$ for the free Boolean algebra on $n$ generators 
  and no relations. 
  Note that $Sp(C_n) = 2^n$ corresponds to the space of finite binary sequences. 
\end{example}
Now we introduce some notation:
\begin{definition}
  \item Given an infinite binary sequence $\alpha:2^\N$ and a natural number $n : \N$  
    we denote $\alpha|_n: 2^n$ for the 
    restriction of $\alpha$ to a finite sequence of length $n$. 
  \item We denote $\overline 0, \overline 1$ 
    for the binary sequences which are constantly $0$ and $1$ respectively. 
  \item We denote $0,1$ for the sequences of length $1$ hitting $0,1$ respectively. 
  \item If $x$ is a finite sequence and $y$ is any sequence, 
    denote $x\cdot y$ for their concatenation. 
\end{definition} 
Now we'll give a definition for when two finite binary sequences of length $n$ correspond 
to real numbers whose distance is $\leq (\frac12)^n$.
Informally, we want for every finite sequence $s$ that 
$(s \cdot 0 \cdot \overline 1)$ and  $(s \cdot 1 \cdot \overline 0)$ are equivalent. 

\begin{definition}
  Let $n:\N$ and let $s,t : 2^n$. 
  We say $s,t$ are $n$-near, and write $s\sim_n t$ if 
  there merely exists some $m:\N$ and some $u:2^m$, such that 
 \begin{equation}\label{EqnNearness}
   \big(
     (s = (u\cdot 0\cdot \overline 1)|_n) \vee (s = (u \cdot 1 \cdot \overline 0) |_n)
   \big)
    \wedge 
   \big(
     (t = (u\cdot 0\cdot \overline 1)|_n) \vee (t = (u \cdot 1 \cdot \overline 0) |_n)
   \big)
  \end{equation} 
\end{definition}
\begin{remark}\label{nearnessProperties}
\item As we're dealing with finite sequences, $s\sim_n t$ is decidable. 
\item Given any $s:2^n$, using $m=n, u = s$ above, we can show that $s\sim_n s$. 
  So $n$-nearness is reflexive. 
\item \Cref{EqnNearness} is symmetric in $s$ and $t$. Hence $n$-nearness is symmetric.
\item Note that $0\cdot 0\sim_2 0\cdot 1 \sim_2 1\cdot 0 \sim_2 1\cdot 1$, 
  but $0\cdot 0\nsim_2 1\cdot 1$. %is not $2$-near to $1\cdot 1$. 
  Thus $n$-nearness is not in general transitive. 
\end{remark}
\begin{definition}
  Let $\alpha, \beta: 2^\N$, we define $a\sim_I\beta$ as 
  $\forall_{n:\N} (\alpha|_n \sim_n \beta|_n)$. 
\end{definition}
\begin{lemma}\label{IntervalFiberSizeAtMost2}
  Whenever $\alpha,\beta,\gamma:2^\N$, are such that 
  $\alpha\sim_I \beta, \beta\sim_I \gamma$, 
  at least two of $\alpha,\beta,\gamma$ are equal. 
\end{lemma}
\begin{proof}
  We will show that $\beta = \gamma \vee \alpha = \gamma \vee \alpha = \beta$. 
  By \Cref{StoneEqualityClosed} and \Cref{ClosedFiniteDisjunction}, this is a closed proposition. 
  By \Cref{rmkOpenClosedNegation}, we can instead show the double negation. 
  To this end, assume that none of $\alpha,\beta,\gamma$ are equal. 
  By \Cref{MarkovPrinciple}, there exist indices $i,j,k\in \N$ with 
  \begin{equation}
    \beta(i) \neq \gamma(i), \alpha(j) \neq \gamma(j), \alpha(k) \neq \beta(k)
  \end{equation}
  Let $n:=\max(i,j,k) + 2$. 
  As $\alpha\sim_I \beta$, we have $\alpha|_n\sim_n\beta|_n$. 
  By assumption $\alpha|_n \neq \beta|_n$, so WLOG we may assume that 
  we have some $m: \N, u:2^m$ with 
  \begin{equation}
    \alpha|_n = (u\cdot 0 \cdot \overline 1) |_n , \beta|_n = (u \cdot 1 \cdot \overline 0)|_n.
  \end{equation}
  As $\alpha(k) \neq \beta(k) $ and $n\geq k+2$, 
  it follows in particular that $m\leq n-2$ and hence 
  $\beta(n-1) = 0$.% and $\beta(m) = 1$. 

  As also $\beta\sim_I \gamma$, we have $\beta|_n \sim_n \gamma|_n$.
  So there exists some $m':\N, u':2^m$ with 
 \begin{equation} %\label{EqnNearness}
   \big(
     (\beta|_{n} = (u'\cdot 0\cdot \overline 1)|_n) \vee (\beta|_{n} = (u' \cdot 1 \cdot \overline 0) |_n)
   \big)
    \wedge 
   \big(
     (\gamma|_{n} = (u'\cdot 0\cdot \overline 1)|_n) \vee (\gamma|_{n} = (u' \cdot 1 \cdot \overline 0) |_n)
   \big).
  \end{equation} 
  Similarly as above, we have that $m'\leq n-2$, and as $\beta(n-1) = 0$, it follows that 
  $\beta|_{n} = (u' \cdot 1 \cdot \overline 0) |_n$. 
  Now as $\beta(i)\neq \gamma(i)$ with $i<n$, we have that $\beta|_n \neq \gamma|_n$, hence 
  $\gamma|_{n} = (u'\cdot 0\cdot \overline 1)|_n$. 
  Now we have $m,m'\leq n-2$ and $u:2^m, u':2^{m'}$ such that 
  \begin{equation}
    (u\cdot 1 \cdot \overline 0)|_n = \beta|_n = (u'\cdot 1 \cdot \overline 0)|_n
  \end{equation}
  Note that $\beta(m') = 1$. 
  But also $\beta(l) = 0$ for all $l$ with $m<l<n$
  Therefore $m'\leq m$. 
  By similar reasoning, $m\leq m'$. We conclude $m=m'$. 
  As a consequence, $u = u'$, but then 
  $\gamma|_n = \alpha|_n$, contradicting that $\alpha(j)\neq \gamma(j) $ for $j<n$. 
  Hence we arrive at a contradiction, as required. 
\end{proof}


\begin{corollary}
  $\sim_I$ is a closed equivalence relation on $2^\N$. 
\end{corollary}
\begin{proof}
  By \Cref{nearnessProperties}, $\sim_I$ is a countable conjunction of decidable propositions. 
  Also by \Cref{nearnessProperties}, $\sim_n$ is reflexive and symmetric for all $n:\N$, thus
  $\sim_I$ is reflexive and symmetric as well. 
  Finally $\sim_I$ is transitive as a consequence of \Cref{IntervalFiberSizeAtMost2}.
\end{proof}
\begin{definition}
  We define $\I:\Chaus$ as $\I= 2^\N/\sim_I$. 
\end{definition}
%------------------
%\input{AllFunctionsAreContinuous}

%\input{Interval/EquivalenceOfSims}
%\input{Interval/Surjective}


%
%
%
%\begin{theorem}
%  The interval of Cauchy reals is isomorphic to $2^\N / \sim_t$. 
%\end{theorem} 
%\begin{proof}
%  This follows from the fact that $b:2^\N$ is such that $\alpha\sim_n \beta$ iff $b(\alpha)\sim_t b(\beta)$. 
%  and for every Cauchy real, there is a binary sequence being sent to it, so the composition of $b$ and the 
%  quotient from Caucy sequences to Cauchy real is a surjection. 
%\end{proof}
%
%\begin{corollary}
%  The interval is compact Hausdorff. 
%\end{corollary}

